A characterization of sample adaptivity in UCB data

We characterize a joint CLT of the number of pulls and the sample mean reward of the arms in a stochastic two-armed bandit environment under UCB algorithms. Several implications of this result are in place: (1) a nonstandard CLT of the number of pulls hence pseudo-regret that smoothly interpolates between a standard form in the large arm gap regime and a slow-concentration form in the small arm gap regime, and (2) a heuristic derivation of the sample bias up to its leading order from the correlation between the number of pulls and sample means. Our analysis framework is based on a novel perturbation analysis, which is of broader interest on its own.

==> proof_sketch.tex <==
\subsection{Technical overview}\label{sec: tech_overview}
% \yc{I reorganized this section.}
We introduce a novel analysis framework to establish our main results, that views the bandit process as a complex dynamical system, and conducts perturbation analysis on top of it. The approach is generic and broadly applicable, of which we provide an overview within the $K$-armed bandit system and for UCB-type algorithms with general index functions $I(\cdot)$. 


\paragraph{A Perturbation Analysis} Generally, any index policy such as {\sf UCB1} adaptively selects the next arm $i$ to pull based on the highest index $I(\bar\mu_{i,t},N_{i,t},t)$ for some index function $I(\cdot)$. In a continuous-time fluid approximation, we replace the stochastic reward by its mean, and let the index policy to continuously pull the arm with the highest index. If $I$ is smooth and satisfies the natural exploration-encouraging conditions (i.e., for any arm in the fluid system, the index increases in time $t$ whenever it is \textit{not} pulled, and decreases otherwise), then all arms' indices will always be kept equal under the algorithm. This gives the following natural characterization of the fluid system (at time $T$):
\begin{align}\label{eq: fluid system}
     I\left(\mu_1, n_{1, T}, T\right) &= I\left(\mu_k, n_{k, T}, T\right),\ \ 2\leq k \leq K\nonumber\\
     \sum_{k = 1}^K n_{k, T} &= T.
\end{align} 


% We introduce a novel analysis framework used to establish our main results, that first approximates the complex bandit dynamics via a fluid system, and then conducts a perturbation analysis on top of it. The approach is generic and broadly applicable, of which we provide an overview within the $K$-armed bandit system and for UCB-type algorithms with general index functions.
%Bandit processes often exhibit complex dynamics, due to the inherent non-stationarity of the learning process, and the full adaptivity of the adaptive allocation algorithms. We introduce a perturbation analytical approach that effectively approximates the dynamics of bandit process under {\sf UCB} algorithms, which forms the foundational framework for a variety of theoretical results presented in the following sections. We provide a high-level overview of this approach in this section.



% \paragraph{Fluid System.} Generally, any index policy such as {\sf UCB1} adaptively selects the next arm $i$ to pull based on the highest index $I(\bar\mu_{i,t},N_{i,t},t)$ for some index function $I(\cdot)$. In a continuous-time fluid approximation, we replace the stochastic reward by its mean, and let the index policy to continuously pull the arm with the highest index. If $I$ is smooth and satisfies the natural exploration-encouraging conditions (i.e., for any arm in the fluid system, the index increases in time $t$ whenever it is \textit{not} pulled, and decreases otherwise), then all arms' indices will always be kept equal under the algorithm. This gives the following natural characterization of the fluid system (at time $T$):
% \begin{align}\label{eq: fluid system}
%      I\left(\mu_1, n_{1, T}, T\right) &= I\left(\mu_k, n_{k, T}, T\right),\ \ 2\leq k \leq K\nonumber\\
%      \sum_{k = 1}^K n_{k, T} &= T.
% \end{align} 
%A natural first step to analyze a complex system's dynamic is to characterize its \textit{fluid approximation}. Consider the continuous-time fluid bandit problem where the reward sequence of each arm $k$ is replaced by a continuous-time process living in $[0, T]$ with a constant rate $\mu_k$. For any fixed index function $I$, there is a natural continuous-time analogy of Algorithm \ref{algo:index-based} which continuously selects the arm with the highest index in the fluid bandit problem. Suppose that $I$ is smooth and satisfies the natural exploration-encouraging conditions: $(i)\ \frac{\partial I(\mu, n, t)}{\partial t} > 0$; and $(ii)\  \frac{\partial I(\mu, n, t)}{\partial t} + \frac{\partial I(\mu, n, t)}{\partial n} < 0$. In other words, for any arm in the fluid system, the index increases in time $t$ whenever it is \textit{not} pulled, and decreases otherwise. Then the fluid system's dynamic driven by the continous-time version of {\sf UCB} can be explicitly characterized through the following equations 
%\begin{definition}[The fluid system of equations]\label{def: fluid system}
%For $t \in [0, T]$,
%\begin{align}\label{eq: fluid system}
%     I\left(\mu_1, n_{1, t}, t\right) &= I\left(\mu_k, n_{k, t}, t\right),\ \ 2\leq k \leq K\nonumber\\
%     \sum_{k = 1}^K n_{k, t} &= t.
%\end{align} 
%\end{definition}
Intuitively, the solution to the above system of equations, denoted by $\bn^{\star}_T \triangleq \left(n^{\star}_{1, T}, \dots n^{\star}_{K, T}\right)$ is expected to be a first-order approximation of $(N_{1,T},...,N_{K,T})$, the true number of pulls, under proper conditions, as observed and formalized in earlier works \cite{kalvit2021closer, han2024ucb}. We refer to $n^{\star}_{1, T}, \dots n^{\star}_{K, T}$ as the \textit{fluid approximation} of the number of pulls of each arm.

This work goes beyond \eqref{eq: fluid system}, and reveals how the true system’s dynamics deviate from the fluid approximation through a perturbation analysis. Inspired by the system of equations \eqref{eq: fluid system}, a natural conjecture is that the {\sf UCB} algorithm in the true system also tries to ``equate the indices''. %\jl{In the fixed point equations, the indices should use $\bar\mu_{i,t-1}$ and $N_{i,t-1}$ in order to be precise. Also $\sum_{k = 1}^T N_{k, t} = t$ should be $\sum_{k = 1}^T N_{k, t-1} = t-1$. Will the proof be affected much? If yes then we should find a way to justify using $\bar\mu_{i,t}$ and $N_{i,t}$ here is a good approximation. Similar for Definition 1 and 2.} 
\begin{conj}[Informal]\label{conj: true system}
In a ``reasonable'' bandit model and under a ``reasonable'' {\sf UCB} algorithm with index function $I$, the number of pulls $N_{k, T}$ should satisfy
\begin{align}\label{eq: true system conjectured fixed point equation}
    I\left(\bar\mu_{1, T}, N_{1, T}, T\right) &\approx  I\left(\bar\mu_{k, T}, N_{k, T}, T\right),\ \ 2\leq k \leq K,\nonumber\\
    \sum_{k = 1}^T N_{k, T} &= T.
\end{align} 
\end{conj}
Replace $I(\cdot)$ by their first-order approximations at $(\mu_k, n^{\star}_{k, T})$, namely
\begin{align*}
% \label{eq: conj-taylor-expansion of index}
    I\left(\bar\mu_{k, T}, N_{k, T}, T\right) \approx I\left(\mu_{k}, n^{\star}_{k, T}, T\right) + I'_{k, 1} \cdot (\underbrace{\bar\mu_{k, T} - \mu_k}_{\bar\Delta_k}) + I'_{k, 2} \cdot (\underbrace{N_{k, T} - n^{\star}_{k, T}}_{\omega_k}),
\end{align*}
where $I'_{k, 1}, I'_{k,2}$ are the partial derivatives of $I$ w.r.t. the first and second arguments evaluated at $(\mu_k,n^{\star}_{k,T},T)$, respectively. This approximation, combined with \eqref{eq: fluid system}, allows us to further simplify the conjectured system of equations \eqref{eq: true system conjectured fixed point equation}, to a system of linear equations
\begin{align*}
    \begin{bmatrix}
1 & 1 & 1 & \dots & 1 \\
-I'_{1,2} & I'_{2,2} & 0 & \dots & 0 \\
\dots  & \dots  & \dots  & \dots & \dots  \\
-I'_{1,2} & 0 & 0 & \dots & I'_{K,2}
\end{bmatrix}
\begin{bmatrix}
\omega_1 \\ \omega_2 \\ \dots \\ \omega_K
\end{bmatrix}
=
\begin{bmatrix}
0 \\ I'_{1,1}\bar\Delta_1  - I'_{2,1}\bar\Delta_2 \\ \dots \\ I'_{1, 1}\bar\Delta_1 - I'_{K,1}\bar\Delta_K
\end{bmatrix}.
\end{align*}
which admits closed-form solutions (Refer to Appendix \ref{app:k-arm} for a precise form). In particular, we obtain approximations of $N_{k, T}, k = 1, \dots K$ beyond their fluid approximations $\bn^{\star}_T$, each as an linear combination of the sample means $\bar\mu_{k, T}, k = 1, \dots K$. This characterizes the dependence structure between $N_{k, T}$ and $\bar\mu_{k, T}$ for $k = 1, \dots K$. We then arrive at the joint CLT of \eqref{eq:main-result-informal} (and Theorem \ref{thm:N1}) through an approximation of each $\bar\mu_{k, T}$ by the sample means of the corresponding arm at their fluid approximation $n^{\star}_{k, T}$, which are non-adaptive, completely independent and asymptotically normal across arms $k = 1, \dots, K$.

The main result of this work, Theorem \ref{thm:N1}, can be viewed as a formalization of the above intuition in the two-arm case, with the ``reasonable'' bandit model, the ``reasonable'' {\sf UCB} algorithm, as well as the precise notion of ``approximately equal'' rigorously specified. We expect that similar results hold in the general $K$-arm setting. A precise form of the joint CLT, derived following the procedures sketched above, is provided in Appendix~\ref{app:k-arm}, with brief discussion of its implications, although a formal proof is omitted. We expect the analysis to be similar to the two-arm setting.

% Plugging back to (\ref{eq: true system conjectured fixed point equation}) effectively yields $N_{k, T}$, each in the form of an affine function of the sample means $\bar\mu_{k, T}, k = 1, \dots K$. This characterizes the dependence structure between $N_{k, T}$ and $\bar\mu_{k, T}$ for $k = 1, \dots K$. We then arrive at the joint CLT of \eqref{eq:main-result-informal} (and Theorem \ref{thm:N1}) through an approximation of each $\bar\mu_{k, T}$ by the sample means of the corresponding arm at their fluid approximation $n^{\star}_{k, T}$, which are non-adaptive, completely independent and asymptotically normal across arms $k = 1, \dots, K$. 


% The main result of this work, Theorem \ref{thm:N1}, can be viewed as a formalization of Conjecture \ref{conj: true system}, with the ``reasonable'' bandit model, the ``reasonable'' {\sf UCB} algorithm, as well as the precise notion of ``approximately equal'' rigorously specified. We provide an informal, yet intuitive roadmap. Note that the system of equations \eqref{eq: true system conjectured fixed point equation} can be further simplified through a first-order approximation performed at the fluid approximation
% \begin{align}\label{eq: conj-taylor-expansion of index}
%     I\left(\bar\mu_{k, T}, N_{k, T}, T\right) \approx  I'_1 \cdot \left(\bar\mu_{k, T} - \mu_k\right) + I'_2 \cdot \left(N_{k, T} - n^{\star}_{k, T}\right) + I\left(\mu_{k}, n^{\star}_{k, T}, T\right),
% \end{align}
% with $I'_1, I'_2$ the partial derivatives w.r.t. the first and second arguments evaluated at $(\mu_k,n^{\star}_{k,T},T)$, respectively.
% \jl{partial derivatives w.r.t. the first and second arguments evaluated at $(\mu_k^T,n^{\star}_{k,T},T)$?}.
 

%One intuitive interpretation of equations (\ref{eq: fluid system}) is that the {\sf UCB} algorithm always maintains a balance among all arms by equating their indices. Denote by $\bn^{\star}_t \triangleq \left(n^{\star}_{1, t}, \dots n^{\star}_{K, t}\right)$ the solution to the above system of equations at $t \in [0, T]$. We shall refer to $\bn^{\star}_T$ as the \textit{fluid approximation} of the number of pulls of each arm. Under certain conditions, $\bn^{\star}_T$ is a set of asymptotically good approximation of $\bN_T$, namely the number of pulls under Algorithm \ref{algo:index-based} in the true system (see Section \ref{sec: assumption}).


% Under certain conditions, prior work \citep{kalvit2021closer, han2024ucb} established that $\bn^{\star}_T$ is a set of asymptotically good approximation of $\bN_T$, namely the number of pulls under Algorithm \ref{algo:index-based} in the true system (see Section \ref{sec: assumption}), and this serves as the starting point of our perturbation analysis.



% \paragraph{A Perturbation Analysis.} We develop technical tools that characterize how the true system’s dynamics deviate from the fluid approximation. Inspired by the system of equations \eqref{eq: fluid system}, a natural conjecture is that the {\sf UCB} algorithm in the true system also tries to ``equate the indices''. %\jl{In the fixed point equations, the indices should use $\bar\mu_{i,t-1}$ and $N_{i,t-1}$ in order to be precise. Also $\sum_{k = 1}^T N_{k, t} = t$ should be $\sum_{k = 1}^T N_{k, t-1} = t-1$. Will the proof be affected much? If yes then we should find a way to justify using $\bar\mu_{i,t}$ and $N_{i,t}$ here is a good approximation. Similar for Definition 1 and 2.} 
% \begin{conj}[Informal]\label{conj: true system}
% In a ``reasonable'' bandit model and under a ``reasonable'' {\sf UCB} algorithm with index function $I$, the number of pulls $N_{k, T}$ should satisfy
% \begin{align}\label{eq: true system conjectured fixed point equation}
%     I\left(\bar\mu_{1, T}, N_{1, T}, T\right) &\approx  I\left(\bar\mu_{k, T}, N_{k, T}, T\right),\ \ 2\leq k \leq K,\nonumber\\
%     \sum_{k = 1}^T N_{k, T} &= T.
% \end{align} 
% \end{conj}
% The main result of this work, Theorem \ref{thm:N1}, can be viewed as a formalization of Conjecture \ref{conj: true system}, with the ``reasonable'' bandit model, the ``reasonable'' {\sf UCB} algorithm, as well as the precise notion of ``approximately equal'' rigorously specified. We first provide an informal, yet intuitive roadmap. Note that the system of equations \eqref{eq: true system conjectured fixed point equation} can be further simplified through a first-order approximation performed at the fluid approximation
% \begin{align}\label{eq: conj-taylor-expansion of index}
%     I\left(\bar\mu_{k, T}, N_{k, T}, T\right) \approx  I'_1 \cdot \left(\bar\mu_{k, T} - \mu_k\right) + I'_2 \cdot \left(N_{k, T} - n^{\star}_{k, T}\right) + I\left(\mu_{k}, n^{\star}_{k, T}, T\right),
% \end{align}
% with $I'_1, I'_2$ the partial derivatives w.r.t. the first and second arguments evaluated at $(\mu_k,n^{\star}_{k,T},T)$, respectively.
% % \jl{partial derivatives w.r.t. the first and second arguments evaluated at $(\mu_k^T,n^{\star}_{k,T},T)$?}.
% Plugging back to (\ref{eq: true system conjectured fixed point equation}) effectively yields $N_{k, T}$, each in the form of an affine function of the sample means $\bar\mu_{k, T}, k = 1, \dots K$. This characterizes the dependence structure between $N_{k, T}$ and $\bar\mu_{k, T}$ for $k = 1, \dots K$. We then arrive at the joint CLT of \eqref{eq:main-result-informal} (and Theorem \ref{thm:N1}) through an approximation of each $\bar\mu_{k, T}$ by the sample means of the corresponding arm at their fluid approximation $n^{\star}_{k, T}$, which are non-adaptive, completely independent and asymptotically normal across arms $k = 1, \dots, K$. 

% The proof of Theorem~\ref{thm:N1} requires us to rigorously formalize each of the approximations made in the above intuitive derivation. In particular, within the setting $K = 2$ and under the index algorithm of a UCB form, the existence of an arm $i$ receiving an exceptionally large number of arm pulls $N_{i, T} > a$ necessarily implies that there exists time $t \leq T$ such that arm $i$ with index $\bamu_i(a)+ \frac{f(t)}{\sqrt{a}}$ gets selected over the other arm with index $\bamu_{-i}(t - a) + \frac{f(t)}{\sqrt{t - a}}$ (we denote $-i$ the index of the arm that is not $i$, and denote $\bamu_i(a)$ the sample mean of arm $i$'s first $a$ collected rewards, i=1,2). We then prove that the probability of existing a time $t\leq T$ such that $\bamu_{-i}(t - a) + \frac{f(t)}{\sqrt{t - a}}$ is smaller than $\bamu_i(a)+ \frac{f(t)}{\sqrt{a}}$ vanishes with $T \to \infty$, where $a$ is set to be larger by a constant $\epsilon$ than the ``predicted value'' of $N_{i, T}$ as an affine function of the sample means (after proper normalization), derived from solving \eqref{eq: true system conjectured fixed point equation} 
% %\jl{can't parse this sentence}, i.e. the affine function of the sample means. 
% This proves \eqref{eq: true system conjectured fixed point equation} holds in a high probability sense. A crucial bounding technical in treating the above probability is to treat two cases differently: (i) such $t$ exists and $t \in [\tau_T, T]$, and (ii)  such $t$ exists and is smaller than $\tau_T$, where $\tau_T$ is a properly chosen threshold. We use the fact that in (i), the approximation of \eqref{eq: conj-taylor-expansion of index} is tight enough, and the two sample means $\bamu_{i}(a), \bamu_{-i}(t - a)$ are close to $\bamu_{i}(n^{\star}_{i, T}), \bamu_{-i}(n^{\star}_{-i, T})$ due to a strong high-probability contraction guarantee of a random walk's running sample means (cf. Lemma \ref{lem: maximal inequality}); and in (ii), $t$ is so small that $\frac{f(t)}{\sqrt{t - a}}$ necessarily dominates, and makes the index of $-i$ the larger one across all $t \geq \tau_T$ with high probability. Bounding the probability of events in both these cases essentially boils down to various probability bounds on random walk large deviation. With the dependence structure characterized 
%  in \eqref{eq: true system conjectured fixed point equation} proved, the proof of the ultimate joint CLT is relatively straightforward. 

